ARMA Nets: Expanding Receptive Field for Dense Prediction

Global information is essential for dense prediction problems, whose goal is to compute a discrete or continuous label for each pixel in the images. Traditional convolutional layers in neural networks, initially designed for image classification, are restrictive in these problems since the filter size limits their receptive fields. In this work, we propose to replace any traditional convolutional layer with an autoregressive moving-average (ARMA) layer, a novel module with an adjustable receptive field controlled by the learnable autoregressive coefficients. Compared with traditional convolutional layers, our ARMA layer enables explicit interconnections of the output neurons and learns its receptive field by adapting the autoregressive coefficients of the interconnections. ARMA layer is adjustable to different types of tasks: for tasks where global information is crucial, it is capable of learning relatively large autoregressive coefficients to allow for an output neuron's receptive field covering the entire input; for tasks where only local information is required, it can learn small or near zero autoregressive coefficients and automatically reduces to a traditional convolutional layer. We show both theoretically and empirically that the effective receptive field of networks with ARMA layers (named as ARMA networks) expands with larger autoregressive coefficients. We also provably solve the instability problem of learning and prediction in the ARMA layer through a re-parameterization mechanism. Additionally, we demonstrate that ARMA networks substantially improve their baselines on challenging dense prediction tasks including video prediction and semantic segmentation.

==> figures/ablation_acc/AblationStudy-VGG-no-reparam-ACC.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.97,0.03)}, anchor=south east, draw=white!80!black},
tick align=outside,
tick pos=both,
title={Ablation Study ACC},
x grid style={white!69.0196078431373!black},
xlabel={epoch},
xmin=-14.95, xmax=313.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={ACC},
ymin=0.00343518379407051, ymax=0.00653389172676282,
ytick style={color=black}
]
\addplot [semithick, red]
table {%
0 0.00357603415464744
1 0.0042568108974359
2 0.00482412484975962
3 0.00538752629206731
4 0.00534448868189103
5 0.00577486478365385
6 0.00636956630608974
7 0.00555967673277244
8 0.00583355243389423
9 0.00527015099158654
10 0.00590006510416667
11 0.00533666366185897
12 0.00611134064503205
13 0.00532883864182692
14 0.00590006510416667
15 0.00504713792067308
16 0.00572400215344551
17 0.00498845027043269
18 0.00541882637219551
19 0.00528188852163462
20 0.00515668820112179
21 0.00579833984375
22 0.00487498747996795
23 0.00499236278044872
24 0.00521928836137821
25 0.00538752629206731
26 0.00505887545072115
27 0.00531318860176282
28 0.00515668820112179
29 0.00509017553084936
30 0.00511756310096154
31 0.00552837665264423
32 0.00494150015024038
33 0.00477717472956731
34 0.00559097681290064
35 0.00490628756009615
36 0.00523493840144231
37 0.00546968900240385
38 0.00523102589142628
39 0.00539535131209936
40 0.00495715019030449
41 0.00451503655849359
42 0.00449156149839744
43 0.00458937424879808
44 0.00404944786658654
45 0.0048984625400641
46 0.0048828125
47 0.00451894906850962
48 0.00416291065705128
49 0.00507061298076923
50 0.00411596053685897
51 0.00386164738581731
52 0.00421768579727564
53 0.00455024914863782
54 0.00444852388822115
55 0.00448373647836538
56 0.00454242412860577
57 0.00438983623798077
58 0.00509017553084936
59 0.00479673727964744
60 0.00419421073717949
61 0.00464806189903846
62 0.00472239958934295
63 0.00397119766626603
64 0.00412769806690705
65 0.005035400390625
66 0.00426072340745192
67 0.00476934970953526
68 0.00518016326121795
69 0.0047145745693109
70 0.00498845027043269
71 0.003662109375
72 0.00404944786658654
73 0.00437027368790064
74 0.00395554762620192
75 0.00474196213942308
76 0.00487498747996795
77 0.00455024914863782
78 0.00396337264623397
79 0.00435071113782051
80 0.00462067432892628
81 0.00474978715945513
82 0.00428419846754808
83 0.00402206029647436
84 0.00469892452924679
85 0.00471848707932692
86 0.00408074794671474
87 0.00491020007011218
88 0.00452286157852564
89 0.00491802509014423
90 0.00479673727964744
91 0.00493758764022436
92 0.00419029822716346
93 0.00484759990985577
94 0.00449156149839744
95 0.00434288611778846
96 0.00501583784054487
97 0.00529753856169872
98 0.00497671274038462
99 0.00519972581129808
100 0.00471848707932692
101 0.00460502428886218
102 0.00473804962940705
103 0.00510973808092949
104 0.00490237505008013
105 0.0045932867588141
106 0.00469109950921474
107 0.00406509790665064
108 0.00483194986979167
109 0.00456981169871795
110 0.0048828125
111 0.00474196213942308
112 0.00451112404847756
113 0.00462067432892628
114 0.00417073567708333
115 0.0047458746494391
116 0.00489455003004808
117 0.00461676181891026
118 0.0047458746494391
119 0.00436636117788462
120 0.00382643479567308
121 0.00512930063100962
122 0.00462067432892628
123 0.00449938651842949
124 0.00480847480969551
125 0.00462849934895833
126 0.00468718699919872
127 0.00376383463541667
128 0.00422159830729167
129 0.00516842573116987
130 0.00391642252604167
131 0.00461676181891026
132 0.00483586237980769
133 0.00523885091145833
134 0.00555967673277244
135 0.00510973808092949
136 0.00401423527644231
137 0.00433506109775641
138 0.00428028595753205
139 0.0044406988681891
140 0.00445634890825321
141 0.00382252228565705
142 0.00428028595753205
143 0.00475369966947115
144 0.00379122220552885
145 0.0039516351161859
146 0.00435071113782051
147 0.00428028595753205
148 0.00474196213942308
149 0.00523102589142628
150 0.0048984625400641
151 0.00490628756009615
152 0.00500018780048077
153 0.00513712565104167
154 0.00520755083133013
155 0.00527406350160256
156 0.00519972581129808
157 0.00528188852163462
158 0.00516060071113782
159 0.00523493840144231
160 0.00522711338141026
161 0.00524667593149038
162 0.00496497521033654
163 0.00544230143229167
164 0.00530145107171474
165 0.00547360151241987
166 0.00552446414262821
167 0.00546968900240385
168 0.00572791466346154
169 0.00557141426282051
170 0.00548533904246795
171 0.00528580103165064
172 0.00552055163261218
173 0.00538361378205128
174 0.00565748948317308
175 0.00568878956330128
176 0.00552446414262821
177 0.00586094000400641
178 0.00559097681290064
179 0.00585311498397436
180 0.00568487705328526
181 0.00575138972355769
182 0.0059665777744391
183 0.00580225235376603
184 0.00572400215344551
185 0.00559488932291667
186 0.00573965219350962
187 0.00572400215344551
188 0.00565357697315705
189 0.00582572741386218
190 0.00563401442307692
191 0.00555576422275641
192 0.00591180263421474
193 0.00600570287459936
194 0.00581790239383013
195 0.00592745267427885
196 0.00579051482371795
197 0.00592354016426282
198 0.00572400215344551
199 0.00580616486378205
200 0.00596266526442308
201 0.00577877729366987
202 0.00591962765424679
203 0.00579833984375
204 0.00603700295472756
205 0.00584528996394231
206 0.00566922701322115
207 0.00618567833533654
208 0.00588050255408654
209 0.00594701522435897
210 0.00574747721354167
211 0.00591962765424679
212 0.00589615259415064
213 0.00562227689302885
214 0.00590006510416667
215 0.00604874048477564
216 0.00608395307491987
217 0.00607612805488782
218 0.00609177809495192
219 0.00599396534455128
220 0.00607221554487179
221 0.00602135291466346
222 0.00609569060496795
223 0.00606047801482372
224 0.00609960311498397
225 0.00610742813501603
226 0.00609960311498397
227 0.00605265299479167
228 0.0061191656650641
229 0.00611525315504808
230 0.00613090319511218
231 0.00609177809495192
232 0.00608004056490385
233 0.0061191656650641
234 0.00617785331530449
235 0.0062717535556891
236 0.00609177809495192
237 0.00614264072516026
238 0.00611134064503205
239 0.00619741586538462
240 0.00618567833533654
241 0.00628349108573718
242 0.00611134064503205
243 0.00616220327524038
244 0.00620132837540064
245 0.00614655323517628
246 0.00617785331530449
247 0.00609569060496795
248 0.0062404534755609
249 0.00609569060496795
250 0.00626001602564103
251 0.00615046574519231
252 0.00616611578525641
253 0.00623262845552885
254 0.00624436598557692
255 0.00619741586538462
256 0.00624436598557692
257 0.00621306590544872
258 0.00606830303485577
259 0.00631087865584936
260 0.00620524088541667
261 0.00618959084535256
262 0.00620524088541667
263 0.00629131610576923
264 0.00621306590544872
265 0.00622871594551282
266 0.00634217873597756
267 0.00617785331530449
268 0.00621697841546474
269 0.00618176582532051
270 0.00628740359575321
271 0.00620524088541667
272 0.00624827849559295
273 0.00636565379607372
274 0.00619350335536859
275 0.0062404534755609
276 0.00623262845552885
277 0.00627957857572115
278 0.00621697841546474
279 0.00633435371594551
280 0.00625219100560897
281 0.00626784104567308
282 0.00626784104567308
283 0.00636565379607372
284 0.00626001602564103
285 0.00630305363581731
286 0.00633435371594551
287 0.00628349108573718
288 0.0062717535556891
289 0.00624436598557692
290 0.00622480343549679
291 0.0063930413661859
292 0.00626001602564103
293 0.00621306590544872
294 0.00620915339543269
295 0.00636565379607372
296 0.00626784104567308
297 0.00631479116586538
298 0.00633826622596154
299 0.00631479116586538
};
\addlegendentry{acc}
\end{axis}

\end{tikzpicture}


==> figures/ablation_acc/AblationStudy-VGG-no-reparam-NLL.tex <==
% This file was created by tikzplotlib v0.9.1.
\begin{tikzpicture}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=both,
x grid style={white!69.0196078431373!black},
xlabel={epoch},
xmin=-14.95, xmax=313.95,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={NLL},
ymin=0.000367181598722266, ymax=0.000440235503005962,
ytick style={color=black}
]
\addplot [semithick, blue]
table {%
0 0.000428725740848443
1 0.000415377078864437
2 0.000395264887871842
3 0.000389460983495109
4 0.000391025411394926
5 0.000383202528628783
6 0.000376304090978243
7 0.000384740923674634
8 0.000381907558617875
9 0.000394317587145055
10 0.000384620830822641
11 0.000394031229930428
12 0.000378975133674267
13 0.000394634664870608
14 0.000386334735995684
15 0.000397874006571678
16 0.000389908206983446
17 0.000391694468756517
18 0.000400196310753624
19 0.000396615670970044
20 0.000394001938044452
21 0.00039185289448748
22 0.000414214978137842
23 0.000398094510325255
24 0.000395255704792455
25 0.000397094754645458
26 0.000400796725462453
27 0.000399665187041347
28 0.000399202651057679
29 0.000398102668949809
30 0.000399757734237191
31 0.00039520943358254
32 0.000394002477136942
33 0.000402654927128401
34 0.000393884539460907
35 0.000404202953601877
36 0.00039128808853909
37 0.000390174947320842
38 0.000396057433233811
39 0.00039807725757456
40 0.000408195765712895
41 0.000414054764386935
42 0.000409556236356879
43 0.000406807684339583
44 0.000412965623232035
45 0.00040695214500794
46 0.000410262480951273
47 0.000412435306665989
48 0.000422465169611268
49 0.000402393920991856
50 0.000412301630832446
51 0.000412698895431673
52 0.000424194006392589
53 0.000406267364413883
54 0.000405993477966732
55 0.000406479285671734
56 0.000406733526585576
57 0.000407954937038131
58 0.000405968303601138
59 0.000405171093865274
60 0.00041582781331948
61 0.000402052849769974
62 0.000402435831701717
63 0.000419613690330432
64 0.000413757743528829
65 0.000403313255773332
66 0.000411984976978065
67 0.000400936863241861
68 0.000401361073510578
69 0.00040527211729055
70 0.000405286333093849
71 0.000436914870993067
72 0.000419122024248235
73 0.000411593595830103
74 0.000409317845836855
75 0.000408450808996956
76 0.000404315345729582
77 0.000401648821142048
78 0.000419845925166439
79 0.000407130907003123
80 0.000405107902434583
81 0.000408772928998447
82 0.000412053848282458
83 0.000410912699925785
84 0.000405571405560924
85 0.000404969707895548
86 0.000416550540532439
87 0.0004018048911045
88 0.000405098577268804
89 0.000400476557656358
90 0.000407221341410126
91 0.000408109322261925
92 0.000410788279408828
93 0.000399724546318444
94 0.000409543559026833
95 0.0004089558401551
96 0.000395066940631622
97 0.000400386684430906
98 0.000403588560099403
99 0.000395846076739522
100 0.000405522385158409
101 0.000403598254212202
102 0.00040930146829058
103 0.000402894533740786
104 0.000402651164226998
105 0.000410124007015465
106 0.000415225217763621
107 0.000410825435000543
108 0.000402129067776677
109 0.00040481517282434
110 0.000404406084607427
111 0.000405140346489274
112 0.000411784623821194
113 0.000414220177425215
114 0.000406959692899806
115 0.000402379272959362
116 0.000400600142371005
117 0.000410430252743073
118 0.000420145040903336
119 0.000413930094323288
120 0.000426157845709568
121 0.00040139951922286
122 0.000414828533449998
123 0.000410825189632865
124 0.000407380121163069
125 0.0004053184732747
126 0.000413019649493389
127 0.0004302231177019
128 0.000419175270228432
129 0.000402873091829511
130 0.000421041816186446
131 0.000406469020228355
132 0.000409368356952492
133 0.000404613127764792
134 0.000403874359714488
135 0.000398773468959217
136 0.000419263435432162
137 0.000408454157579213
138 0.000416192731175285
139 0.00041454584361651
140 0.00041655742097646
141 0.000412802860284081
142 0.000418692574096032
143 0.000411129864052129
144 0.000422815894946838
145 0.000414410374390009
146 0.000412668094325524
147 0.000408209479437807
148 0.000407585140484839
149 0.000402142025100497
150 0.000404633482536062
151 0.000401036712961892
152 0.000400631651521111
153 0.000399666160154037
154 0.00039303402046267
155 0.00039728647396446
156 0.000393251062800678
157 0.000394821872051137
158 0.000395114090030965
159 0.000392408346017011
160 0.000393419775467079
161 0.000392115208057639
162 0.000393496949273424
163 0.0003894619572048
164 0.000390961071930062
165 0.00038806462349991
166 0.000387601420068397
167 0.000387744028837635
168 0.000387539046529967
169 0.00038730603738282
170 0.000388740184000478
171 0.000387968091318049
172 0.000387857056772098
173 0.000386809927220337
174 0.000387079338543117
175 0.000383576762098341
176 0.000385279873481546
177 0.000383670887766549
178 0.000383100179859843
179 0.000382335039261633
180 0.000382750584051395
181 0.000382918485989555
182 0.000381384138614894
183 0.000381393658403212
184 0.000383914504439021
185 0.000382725002530676
186 0.000380327956727109
187 0.000379861097257489
188 0.000386786931910767
189 0.000381672681452563
190 0.000386936381721917
191 0.000381598882496548
192 0.000380891956723271
193 0.000381129565171133
194 0.000384702500648414
195 0.000376678115497224
196 0.000381500442894414
197 0.000382881420545089
198 0.000378914795911465
199 0.000377457901739921
200 0.000377263710834086
201 0.000377326506452683
202 0.000378547636314462
203 0.000376509953266344
204 0.000377929219020865
205 0.000374491659040826
206 0.000378138188105554
207 0.000376645878602106
208 0.00037596043653022
209 0.000374987193693717
210 0.000378358605293891
211 0.000379765755496919
212 0.000379056958123468
213 0.000387158789910758
214 0.000378932038513132
215 0.000378994277129189
216 0.000380056291126097
217 0.000376521597783535
218 0.000379554235424178
219 0.000379545552035173
220 0.000379272907948456
221 0.000380294060764404
222 0.000375544855323357
223 0.000382925333001484
224 0.000374542100307269
225 0.000376712519508333
226 0.000378276951587162
227 0.00037649089936167
228 0.000375007264889204
229 0.000378430370265284
230 0.000377323864123378
231 0.000379237114714506
232 0.000377649056892364
233 0.000375261711171613
234 0.00037687197387314
235 0.000374350260393933
236 0.000377549620297475
237 0.000376288085363996
238 0.000376516029549142
239 0.000375716588221108
240 0.000374388238653923
241 0.000375465002173606
242 0.000376973007447444
243 0.000376926371469521
244 0.000373818899074999
245 0.000373890735686589
246 0.000375493695266927
247 0.000374252925841854
248 0.000373338503189958
249 0.00037724350232822
250 0.000376053904302609
251 0.000376699774120099
252 0.000374202489351424
253 0.000374898287013937
254 0.000375679938289791
255 0.000374103045592514
256 0.000375356067282458
257 0.00037332627002914
258 0.000378369019987682
259 0.000371536964741655
260 0.00037456971521561
261 0.000377741764681653
262 0.000377888744696975
263 0.000373159273742483
264 0.000378734425593836
265 0.00037546394010767
266 0.00037340612258189
267 0.00037581907847944
268 0.000374377380387905
269 0.000375557539220422
270 0.000373731695043926
271 0.000374790293594392
272 0.000373659694853884
273 0.000373909411689219
274 0.000373601334957549
275 0.000375615217340871
276 0.000377851230307267
277 0.000373838345209758
278 0.000373812065794109
279 0.000374422382372312
280 0.000374398320817795
281 0.000374369114900056
282 0.000374442535954026
283 0.000374199583744391
284 0.000374785953392394
285 0.00037486064605988
286 0.000374285165124979
287 0.0003719673706935
288 0.000375600811094046
289 0.000373823764041448
290 0.000374739977698296
291 0.000372760579324304
292 0.000375031808821055
293 0.000375990303328786
294 0.000374551309057726
295 0.000375348839383477
296 0.000374606737078956
297 0.000373507825395045
298 0.000374473498847622
299 0.000370502230735161
};
\addlegendentry{nll}
\end{axis}

\end{tikzpicture}

